Compositional Convolutional Neural Networks: A Robust and Interpretable Model for Object Recognition under Occlusion

Computer vision systems in real-world applications need to be robust to partial occlusion while also being explainable. In this work, we show that black-box deep convolutional neural networks (DCNNs) have only limited robustness to partial occlusion. We overcome these limitations by unifying DCNNs with part-based models into Compositional Convolutional Neural Networks (CompositionalNets) - an interpretable deep architecture with innate robustness to partial occlusion. Specifically, we propose to replace the fully connected classification head of DCNNs with a differentiable compositional model that can be trained end-to-end. The structure of the compositional model enables CompositionalNets to decompose images into objects and context, as well as to further decompose object representations in terms of individual parts and the objects' pose. The generative nature of our compositional model enables it to localize occluders and to recognize objects based on their non-occluded parts. We conduct extensive experiments in terms of image classification and object detection on images of artificially occluded objects from the PASCAL3D+ and ImageNet dataset, and real images of partially occluded vehicles from the MS-COCO dataset. Our experiments show that CompositionalNets made from several popular DCNN backbones (VGG-16, ResNet50, ResNext) improve by a large margin over their non-compositional counterparts at classifying and detecting partially occluded objects. Furthermore, they can localize occluders accurately despite being trained with class-level supervision only. Finally, we demonstrate that CompositionalNets provide human interpretable predictions as their individual components can be understood as detecting parts and estimating an objects' viewpoint.

==> comments.tex <==
\begin{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% START - Angtian Detecion Text
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Detect P3d+
\begin{table*}
	\small
	\centering
	\tabcolsep=0.11cm
	\begin{tabular}{V{2.5}lV{2.5}cV{2.5}c|c|cV{2.5}c|c|cV{2.5}c|c|cV{2.5}cV{2.5}}
		\multicolumn{12}{c}{\textbf{PASCAL3D+ Vehicles Detection under Occlusion}} \\
		\hline
		Foreground Occ. Level					         & \textbf{L0: 0\%} & \multicolumn{3}{cV{2.5}}{\textbf{L1: 20-40\%}} & \multicolumn{3}{cV{2.5}}{\textbf{L2: 40-60\%}} & \multicolumn{3}{cV{2.5}}{\textbf{L3: 60-80\%}} & Mean \\
		\hline
		Background Occ. Level	& L0 & L1 & L2 & L3 & L1 & L2 & L3 & L1 & L2 & L3 & \\    		
		\hline  
		Faster R-CNN           &98.6 &88.2 &87.1 &84.6 &64.6 &60.2 &55.4 &43.0 &34.9 &26.5 &64.3        \\
        Faster R-CNN with reg. &98.2 &90.8 &88.3 &86.4 &76.9 &71.9 &66.4 &59.5 &51.9 &42.0 &73.2        \\
        CA-CompNet via RPN $\omega=0.5$  \\
        CA-CompNet via RPN $\omega=0$    \\
        \hline
        CA-CompNet via BBV $\omega=0.5$   \\
        CA-CompNet via BBV $\omega=0.2$   \\
        CA-CompNet via BBV $\omega=0$       \\
        \hline
	\end{tabular}
	\caption{Detection results on the OccludedVehiclesDetection dataset under different levels of occlusions (BBV means Bounding Box Voting). All models trained on PASCAL3D+3
	unoccluded dataset except Faster R-CNN with reg. was trained with CutOut. The results are measured by mean $AP_{50}$. Notice with $\omega=0.5$, context-aware model reduces to a CompositionalNet.}
    \label{tab:p3d_detection}
\end{table*}

% Detect Coco
\begin{table*}
	\small
	\centering
	\tabcolsep=0.11cm
	\begin{tabular}{V{2.5}lV{2.5}c|c|cV{2.5}c|c|cV{2.5}}
		\multicolumn{7}{c}{\textbf{MS-COCO Vehicles Detection under Occlusion}} \\
		\hline
		Occlusion Level					         &\multicolumn{3}{cV{2.5}}{\textbf{Light Occlusion}} & \multicolumn{3}{cV{2.5}}{\textbf{Heavy Occlusion}}  \\
		\hline
		Average Precision	& $AP$ & $AP_{50}$ & $AP_{75}$ & $AP$ & $AP_{50}$ & $AP_{75}$ \\    		
		\hline  
		Faster R-CNN           &34.6 &69.0 &29.9 &23.0 &28.3 &6.6        \\
		Faster R-CNN with occ. &33.7 &67.5 &30.1 &23.1 &32.7 &7.7        \\
        Faster R-CNN with reg. &41.1 &73.7 &42.3 &28.4 &35.8 &12.6        \\
        CA-CompNet via RPN $\omega=0.5$  \\
        CA-CompNet via RPN $\omega=0$    \\
        \hline
        CA-CompNet via BBV $\omega=0.5$   \\
        CA-CompNet via BBV $\omega=0.2$   \\
        CA-CompNet via BBV $\omega=0$ 

	\end{tabular}
	\caption{Detection results on MS-COCO Dataset. All models are trained on PASCAL3D+ dataset, Faster R-CNN with reg. is trained with cutout and Faster R-CNN with occ. is trained with images in same dataset but occluded by all levels of occlusion with the same set of occluders.}
    \label{tab:coco_detection}
\end{table*}

\begin{itemize}
    \item Scale (with part compositions?)
    \item Multi-Object with non-max suppression?
    \item Better context?
    \item compute numbers for rpn + compnet
\end{itemize}

\subsubsection{Object Detection under Simulated Occlusion}
\todo{introduction of baseline, dataset and problem}
\newline
\todo{result of detection on pascal3D+, (use the result in CVPR), also explain this dataset only have single object (and say we give them the oracle size)}


\subsubsection{Object Detection under Realistic Occlusion}
\todo{put the new result here}
\newline
\todo{Put some images here}
\newline
\todo{explain the method that also us to implement our compositional net to the multi-scale and multi-object image} \newline

In order to evaluate the tested models on real-world occlusions, we evaluated our CompositionalNet on a selected subset of the MS-COCO dataset, We term this dataset \textit{OccludedCOCO}.
In particular, we extract the same classes of objects and scale as in the OccludedVehiclesDetection dataset from the MS-COCO dataset. We select images that contains occluded objects and separate them into two groups: light occlusion and heavy occlusions, with objects under variant occlusions, based on the available segmentation masks. We also manually check and drop those images inside Vehicles or only contains few parts.

This dataset is built from images in both Training2017 and Val2017 set of MSCOCO due to a limited amount of heavily occluded objects in MSCOCO Dataset. The light occlusion set contains 2980 images, the heavy occlusion set contains 756 images.

(refer: Scale Normalization for Image Pyramids)
Due to the variant scale of objects inside this dataset. We proposed a image pyramid for inference. \todo{Check if this could be called image pyramid} To be detail, we resize one target image to multiple scale, by resize the short edge of the image to [300, 370, 460, 580, 720, 1080] without change the ratio of the image. Then we combine the proposals from this image pyramid, by filter out those unreasonable proposals from each re-scaled images and transfer all the proposals to original image. By non-max suppression we could reduce the number of proposals and combine those similar proposals.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% END - Angtian Detecion Text
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Limitations}
\label{sec:exp_limits}
\begin{itemize}
    \item show failure cases in detection, classification, occluder localization, sp detection
\end{itemize}

\subsection{MISC ideas}
\begin{itemize}
    \item Hierarchical Compnets, combine p4+p5, occluder, vcs, classification
    \item Adversarial Robustness?
    \item Object Segmentation?
    \item occluder localization with other architectures
 %   \item integrate context-aware model
%    \item More mixture models (K=32)
%    \item Try E2E on other dataset with p5 (Cifar, imagenet 1000, corrupted mnist), maybe it works
%    \item Consistency in occlusion and mixtures between p4 and p5
%    \item replace vmf with gaussian
%    \item test conv layers instead of max pool layers
\end{itemize}

\end{comment}
